Stein's Lemma for the Reparameterization Trick with Exponential Family Mixtures

Stein's method (Stein, 1973; 1981) is a powerful tool for statistical applications and has significantly impacted machine learning. Stein's lemma plays an essential role in Stein's method. Previous applications of Stein's lemma either required strong technical assumptions or were limited to Gaussian distributions with restricted covariance structures. In this work, we extend Stein's lemma to exponential-family mixture distributions, including Gaussian distributions with full covariance structures. Our generalization enables us to establish a connection between Stein's lemma and the reparameterization trick to derive gradients of expectations of a large class of functions under weak assumptions. Using this connection, we can derive many new reparameterizable gradient identities that go beyond the reach of existing works. For example, we give gradient identities when the expectation is taken with respect to Student's t-distribution, skew Gaussian, exponentially modified Gaussian, and normal inverse Gaussian.

==> content/extension.tex <==
%to do: add this new section this fall.
The following lemma gives a sufficient condition of the smoothness assumption in neural network.
\begin{lemma}
A feedforward neural network is locally ACL with respect to its parameters if all its activation functions are locally Lipschitz-continuous.
\end{lemma}
The proof of this lemma can be readily derived from Theorem 3.1 of \citet{RongQing-notes}.
Unfortunately, the regular chain rule to compute the derivative for a locally ACL function does not hold in general \cite{leoni2007necessary}.
\citet{berner2019towards} discuss a class of piece-wise activation functions where the regular chain rule is valid.
For a general discussion about the chain rule, please see \citet{ambrosio1990general,leoni2007necessary}.


==> content/gn_approx.tex <==
We assume that we want to minimize $\Unmyexpect{q}\sqr{ h(\vlat) }$.
When $q(\vlat)=\gauss(\vlat|\vmu,\vSigma)$, we have
\begin{align}
2 \nabla_\Sigma \Unmyexpect{q}\sqr{ h(\vlat) } &= \Unmyexpect{q}\sqr{ \nabla_\lat^2 h(\vlat) } \\
&= \Unmyexpect{q}\sqr{ \vSigma^{-1} \left(\vlat-\vmu\right) \nabla_\lat h^T(\vlat) }
\end{align}

The key idea is to use control variate such that $\Unmyexpect{q}\sqr{ -\log q(\vlat) }$ is positively correlated to $\Unmyexpect{q}\sqr{ h(\vlat) }$.
The Relax paper exploits a similar idea.
We know that ($\beta >0$)
\begin{align}
 4 \nabla_\Sigma \Unmyexpect{q}\sqr{ h(\vlat) }   + \color{red}{0}
&=  \Unmyexpect{q}\sqr{ \left( \vSigma^{-1} \left(\vlat-\vmu\right) \nabla_\lat h^T(\vlat) \right) + \left( \nabla_\lat h(\vlat) \left(\vlat-\vmu\right)^T \vSigma^{-1} \right)  }
+ 4 \beta \crl{\underbrace{ - \nabla_\Sigma \Unmyexpect{q}\sqr{ -\log q(\vlat) } +  \nabla_\Sigma \Unmyexpect{q}\sqr{ -\log q(\vlat) } }_{0} } \\
&=  \Unmyexpect{q}\sqr{ \left( \vSigma^{-1} \left(\vlat-\vmu\right) \nabla_\lat h^T(\vlat) \right) + \left( \nabla_\lat h(\vlat) \left(\vlat-\vmu\right)^T \vSigma^{-1} \right)  }
+ 4 \beta \crl{\underbrace{ - \nabla_\Sigma \Unmyexpect{q}\sqr{ -\log q(\vlat) } + \half \vSigma^{-1} }_{0} } \\
&=  \Unmyexpect{q}\sqr{ \left( \vSigma^{-1} \left(\vlat-\vmu\right) \nabla_\lat h^T(\vlat) \right) + \left( \nabla_\lat h(\vlat) \left(\vlat-\vmu\right)^T \vSigma^{-1} \right)  }
+ 4 \beta \crl{\underbrace{ - \half  \Unmyexpect{q}\sqr{ \vSigma^{-1} \left(\vlat-\vmu \right) \left(\vlat-\vmu \right)^T \vSigma^{-1} } + \half \vSigma^{-1} }_{0} } 
\end{align} 

For Gauss-Newton approximation ($ \alpha \geq 0$), we have
\begin{align*}
 & \nabla_\Sigma \Unmyexpect{q}\sqr{ h(\vlat) } \\
 =& \frac{1}{2+ 4 \alpha} \left( 4 \alpha\nabla_\Sigma \Unmyexpect{q}\sqr{ h(\vlat) } + 
 \Unmyexpect{q}\sqr{ \nabla_\lat^2 h(\vlat) } \right) \\
 \approx& \frac{1}{2+ 4 \alpha} \left( 4 \alpha\nabla_\Sigma \Unmyexpect{q}\sqr{ h(\vlat) } + 
 \Unmyexpect{q}\sqr{  \nabla_\lat h(\vlat) \nabla_\lat^T h(\vlat) } \right) \\
=&  \frac{1}{2+ 4 \alpha} \Unmyexpect{q}\sqr{ \alpha \sqr{\vSigma^{-1} \left(\vlat-\vmu\right) \nabla_\lat h^T(\vlat)  +   \nabla_\lat h(\vlat) \left(\vlat-\vmu\right)^T \vSigma^{-1}   - 2 \beta \vSigma^{-1} \left(\vlat-\vmu \right) \left(\vlat-\vmu \right)^T \vSigma^{-1}  + 2 \beta \vSigma^{-1} }  + 
   \nabla_\lat h(\vlat) \nabla_\lat^T h(\vlat) }  \\
=&  \frac{1}{2+ 4 \alpha} \Unmyexpect{q}\sqr{ \vw  \vw^T   -  (2\beta \alpha+\alpha^2)  \vSigma^{-1} \left(\vlat-\vmu \right) \left(\vlat-\vmu \right)^T \vSigma^{-1}  + 2 \beta \alpha \vSigma^{-1}       }  
\end{align*} where $\vw=\nabla_\lat h(\vlat) + \alpha \vSigma^{-1} \left(\vlat-\vmu\right)$


==> content/grad_mgm.tex <==
We consider the following Gaussian mean mixture.
\begin{align*}
q(\mix,\vlat|\vmu,\valpha,\vSigma):= &\gauss(\vlat|\vmu+ u(\mix) \valpha,\vSigma) q(\mix) \\
 q(\vlat|\vmu,\valpha,\vSigma) :=& \int q(\mix,\vlat|\vmu,\valpha,\vSigma)  d\mix 
\end{align*}


\begin{theorem}
{\bf Bonnet's Theorem:\\}
Let $h(\vlat):\mathcal{R}^d \mapsto \mathcal{R}$ be a continuous function that satisfies the local ACL property. Furthermore, $\Unmyexpect{q(\lat)}\sqr{\left| \nabla_{\lat_i} h(\vlat) \right|}<\infty$ and $\Unmyexpect{q(\mix,\lat)}\sqr{\left| u(\mix) \nabla_{\lat_i} h(\vlat) \right|}<\infty$  for all $i$, where  $q(\vlat)$ is a Gaussian mean mixture and $q(\mix,\vlat)$ is the joint distribution.
If the regular conditions for Leibniz integral rule are also satisfied, the following gradient identities hold.
\begin{align*}
\nabla_{\mu} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) } =&  \Unmyexpect{q(\lat)}\sqr{ \nabla_{\lat} h(\vlat)}  \\
\nabla_{\alpha} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) } =&  \Unmyexpect{q(\mix,\lat)}\sqr{ u(\mix) \nabla_{\lat} h(\vlat)}  
\end{align*}

\end{theorem}

\begin{proof}
 Let's consider the gradient identity for $\valpha$. By the integral rule, we have
 \begin{align*}
& \nabla_{\alpha} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) } \\
 =& \int  \nabla_{\alpha} q(\vlat|\vmu,\valpha,\vSigma) h(\vlat) d\vlat \\
 =& \int   \int \nabla_{\alpha }\sqr{\underbrace{\gauss(\vlat|\vmu+ u(\mix) \valpha,\vSigma) }_{q(\vlat|\mix)}q(\mix) d\mix} h(\vlat) d\vlat \\
 =& \int   \int \sqr{  u(\mix) \vSigma^{-1} \left( \vlat-\vmu-u(\mix)\valpha  \right) \underbrace{ \gauss(\vlat|\vmu+ u(\mix) \valpha,\vSigma) q(\mix)}_{q(\mix,\vlat)} d\mix} h(\vlat) d\vlat \\
 =& \Unmyexpect{q(\mix,\lat)}\sqr{ u(\mix) \vSigma^{-1} \left( \vlat-\vmu-u(\mix)\valpha  \right) h(\vlat) }
 \end{align*}
 
%Since $h(\vlat)$ has the local ACL property, $h_i(\lat_i):=h(\lat_i,\vlat_{-i})$ is local AC w.r.t. $\lat_i$.
Note that $q(\lat_i|\vlat_{-i},\mix)$ is an univariate Gaussian distribution and $\Unmyexpect{q(\mix,\lat)}\sqr{\left| u(\mix) \nabla_{\lat_i} h(\vlat) \right|}<\infty$.
Using a similar argument as Eq. \eqref{eq:nd_stein_lemma_gauss}, where Lemma \ref{lemma:stein_gauss_mean_1d} is used, we have
\begin{align*}
 & \Unmyexpect{q(\mix,\lat)}\sqr{ u(\mix) \nabla_{\lat_i} h(\vlat)}   \\
 =&\Unmyexpect{q(\mix,\lat_{-i})}\sqr{ u(\mix) \Unmyexpect{q(\lat_i|\mix,\lat_{-i})} \sqr{ \nabla_{\lat_i} h(\vlat) } }\\
 =&\Unmyexpect{q(\mix,\lat_{-i})}\sqr{ u(\mix) \Unmyexpect{q(\lat_i|\mix,\lat_{-i})} \sqr{ \ve_i^T \vSigma^{-1} \left( \vlat-\vmu-u(\mix)\valpha \right) h(\vlat) } }\\
 =&\Unmyexpect{q(\mix,\lat)}\sqr{ u(\mix)  \ve_i^T \vSigma^{-1} \left( \vlat-\vmu-u(\mix)\valpha \right) h(\vlat)  }
\end{align*}
Therefore, we have
\begin{align*}
 \nabla_{\alpha} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) } =
  \Unmyexpect{q(\mix,\lat)}\sqr{ u(\mix) \nabla_{\lat_i} h(\vlat)}  
\end{align*}

Similarly, we can show that
\begin{align*}
\nabla_{\mu} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) } =  \Unmyexpect{q(\mix,\lat)}\sqr{ \nabla_{\lat} h(\vlat)}  =  \Unmyexpect{q(\lat)}\sqr{ \nabla_{\lat} h(\vlat)}  
\end{align*}
\end{proof}

\begin{corollary}
If $u(\mix)$ has the following property, 
\begin{align*}
\int u(\mix) q(\mix,\vlat|\vmu,\valpha,\vSigma) d\mix  = \sum_j^k u_j(\vlat,\vmu,\valpha,\vSigma) \hat{q_j}(\vlat),
\end{align*}  where $\hat{q}_i(\vlat)$ is a (normalized) distribution and $k$ is finite,
the following identity also holds.
\begin{align*}
\nabla_{\alpha} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) } =\sum_{j}^k  \Unmyexpect{\hat{q_j}(\lat)}\sqr{ u_j(\vlat,\vmu,\valpha,\vSigma) \nabla_{\lat} h(\vlat)}  
\end{align*}
\end{corollary}



\begin{example}


A concrete example is the multivariate skew Gaussian distribution.
\begin{align*}
q(\mix,\vlat|\vmu,\valpha,\vSigma):= & \gauss(\vlat|\vmu +  |\mix| \valpha, \vSigma) \gauss(\mix|0,1)  \\
 q(\vlat|\vmu,\valpha,\vSigma) := &  \int q(\mix,\vlat|\vmu,\valpha,\vSigma)  d\mix \\
=&  2 \Phi\left( \frac{ \left( \vlat - \vmu \right)^T \vSigma^{-1} \valpha }{ \sqrt{ 1+\valpha^T\vSigma^{-1}\valpha} } \right)\gauss( \vlat| \vmu, \vSigma+\valpha\valpha^T ) 
\end{align*} where $u(\mix)=|\mix|$.

\begin{comment}
\begin{align}
& q(\vlat|\vmu,\valpha,\vSigma) \\
=&   2 \int_{0}^{+\infty}  \gauss(\mix|0,1)  \gauss(\vlat|\vmu+\mix \valpha,\vSigma)  d\mix  \\
&\text{By grouping terms related to $\mix$ together and completing a Gaussian form for $\mix$, we obtain the following expression} \nonumber \\
=& 2 \int_{0}^{+\infty} \gauss( \mix| \frac{ \left( \vlat - \vmu \right)^T \vSigma^{-1} \valpha }{1+\valpha^T\vSigma^{-1}\valpha} , \left( 1+\valpha^T \vSigma^{-1} \valpha \right)^{-1} )
  \gauss( \vlat| \vmu, \vSigma+\valpha\valpha^T ) d\mix \label{eq:skew_gauss_eq1} \\
=&  2 \Phi\left( \frac{ \left( \vlat - \vmu \right)^T \vSigma^{-1} \valpha }{ \sqrt{ 1+\valpha^T\vSigma^{-1}\valpha} } \right)\gauss( \vlat| \vmu, \vSigma+\valpha\valpha^T ) \label{eq:skew_gauss_eq2}
\end{align} where we move from Eq. \ref{eq:skew_gauss_eq1}  to Eq. \ref{eq:skew_gauss_eq2} using the fact that
\begin{align}
 \int_{0}^{+\infty} \gauss( \mix|u,\sigma^2) d\mix &= \int_{ -u/\sigma }^{+\infty} \gauss( \mix'|0,1) d\mix' \\
 &= 1 - \Phi(-u/\sigma )\\
 &= \Phi(u/\sigma)
\end{align}
\end{comment}


Furthermore, we have
\begin{align*}
  \int |\mix| q(\mix,\vlat|\vmu,\valpha,\vSigma) d\mix 
&=  u_1(\vlat,\vmu,\valpha,\vSigma) \gauss( \vlat| \vmu, \vSigma )  + u_2(\vlat,\vmu,\valpha,\vSigma) q(\vlat|\vmu,\valpha,\vSigma) 
\end{align*} where
$u_1(\vlat,\vmu,\valpha,\vSigma)=\frac{\sqrt{2/\pi} }{ 1+\valpha^T \vSigma^{-1} \valpha   }$ and
$u_2(\vlat,\vmu,\valpha,\vSigma)=\frac{ \left( \vlat - \vmu \right)^T \vSigma^{-1} \valpha }{1+\valpha^T\vSigma^{-1}\valpha}$.

\begin{comment}
\begin{align}
  &\int |\mix| q(\mix,\vlat|\vmu,\valpha,\vSigma) d\mix \\
 =& 2 \int_{0}^{+\infty} \mix \gauss(\vlat|\vmu+\mix\valpha,\vSigma)\gauss(\mix|0,1) d\mix \\
 =& 2 \gauss(\vlat|\vmu,\vSigma) \int_{0}^{+\infty}  \frac{\mix}{\sqrt{2\pi}} \exp\crl{ \left(\vlat-\vmu\right)^T \vSigma^{-1} \valpha \mix - \half \mix^2 \left(1+\valpha^T \vSigma^{-1} \valpha \right) } d\mix \\
 =&  \frac{2}{\sqrt{2\pi}} \gauss(\vlat|\vmu,\vSigma) \int_{0}^{+\infty} \mix   \exp\crl{ \left(\vlat-\vmu\right)^T \vSigma^{-1} \valpha \mix - \half \mix^2 \left(1+\valpha^T \vSigma^{-1} \valpha \right) } d\mix \\
 =&  \frac{2\gauss(\vlat|\vmu,\vSigma) }{\sqrt{2\pi}} \int_{0}^{+\infty} \frac{\sqr{\left(1+\valpha^T\vSigma^{-1}\valpha \right) w - \left(\vlat-\vmu\right)^T\vSigma^{-1}\valpha} + \left(\vlat-\vmu\right)^T\vSigma^{-1}\valpha }{ 1+\valpha^T\vSigma^{-1}\valpha }   \exp\crl{ \left(\vlat-\vmu\right)^T \vSigma^{-1} \valpha \mix - \half \mix^2 \left(1+\valpha^T \vSigma^{-1} \valpha \right) } d\mix \\
 =&  \frac{-\sqrt{2/\pi}  \gauss(\vlat|\vmu,\vSigma)}{1+\valpha^T\vSigma^{-1}\valpha}  \exp\crl{ \left(\vlat-\vmu\right)^T \vSigma^{-1} \valpha \mix - \half \mix^2 \left(1+\valpha^T \vSigma^{-1} \valpha \right) }\Big|_{0}^{+\infty}  + \frac{ \left(\vlat-\vmu\right)^T\vSigma^{-1}\valpha }{ 1+\valpha^T\vSigma^{-1}\valpha } \int_{0}^{\infty} 2 \gauss(\vlat|\vmu+\mix\valpha,\vSigma)\gauss(\mix|0,1) d\mix \\
 =&  \frac{\sqrt{2/\pi}}{ 1+\valpha^T\vSigma^{-1}\valpha} \gauss(\vlat|\vmu,\vSigma)  + \frac{ \left(\vlat-\vmu\right)^T\vSigma^{-1}\valpha }{ 1+\valpha^T\vSigma^{-1}\valpha }  q(\vlat|\vmu,\valpha,\vSigma) 
\end{align}
\end{comment}

\end{example}

\begin{example}
Another example is the multivariate exponentially modified Gaussian distribution.
\begin{align*}
q(\mix,\vlat|\vmu,\valpha,\vSigma):= & \gauss(\vlat|\vmu +  \mix \valpha, \vSigma) \expdist(\mix|1)  \\
 q(\vlat|\vmu,\valpha,\vSigma) := &  \int_{0}^{+\infty} q(\mix,\vlat|\vmu,\valpha,\vSigma)  d\mix \\
=&  \frac{ \sqrt{2\pi}\mathrm{det}\left(2\pi\vSigma \right)^{-\half} }{  \sqrt{\valpha^T \vSigma^{-1}\valpha} } \Phi\left( \frac{ \left( \vlat-\vmu \right)^T \vSigma^{-1} \valpha -1 }{ \sqrt{ \valpha^T \vSigma^{-1} \valpha }  } \right)\exp\crl{  \half\sqr{ \frac{ \left( \left( \vlat-\vmu \right)^T \vSigma^{-1} \valpha -1 \right)^2  }{ \valpha^T \vSigma^{-1} \valpha } - \left(\vlat-\vmu\right)^T \vSigma^{-1} \left(\vlat-\vmu \right)  }  }
\end{align*} where $u(\mix)=\mix$.


\begin{comment}
\begin{align}
& q(\vlat|\vmu,\valpha,\vSigma) \\
=&    \int_{0}^{+\infty}  \expdist(\mix|0,1)  \gauss(\vlat|\vmu+\mix\valpha,\vSigma)  d\mix  \\
&\text{By grouping terms related to $\mix$ together and completing a Gaussian form for $\mix$, we obtain the following expression} \nonumber \\
=& \frac{ \mathrm{det}\left(2\pi\vSigma \right)^{-\half} }{  \sqrt{\frac{\valpha^T \vSigma^{-1}\valpha}{2\pi}} } \int_{0}^{+\infty} \gauss( \mix| \frac{ \left( \vlat - \vmu \right)^T \vSigma^{-1} \valpha-1 }{\valpha^T\vSigma^{-1}\valpha} , \frac{1}{ \valpha^T \vSigma^{-1} \valpha } ) \exp\crl{  \half\sqr{ \frac{ \left( \left( \vlat-\vmu \right)^T \vSigma^{-1} \valpha -1 \right)^2  }{ \valpha^T \vSigma^{-1} \valpha } - \left(\vlat-\vmu\right)^T \vSigma^{-1} \left(\vlat-\vmu \right)  }  }
 d\mix \label{eq:exp_gauss_eq1}\\
=&  \frac{ \sqrt{2\pi}\mathrm{det}\left(2\pi\vSigma \right)^{-\half} }{  \sqrt{\valpha^T \vSigma^{-1}\valpha} } \Phi\left( \frac{ \left( \vlat-\vmu \right)^T \vSigma^{-1} \valpha -1 }{ \sqrt{ \valpha^T \vSigma^{-1} \valpha }  } \right)\exp\crl{  \half\sqr{ \frac{ \left( \left( \vlat-\vmu \right)^T \vSigma^{-1} \valpha -1 \right)^2  }{ \valpha^T \vSigma^{-1} \valpha } - \left(\vlat-\vmu\right)^T \vSigma^{-1} \left(\vlat-\vmu \right)  }  }
 \label{eq:exp_gauss_eq2}
\end{align}
where we move from Eq. \ref{eq:exp_gauss_eq1}  to Eq. \ref{eq:exp_gauss_eq2} using the fact that
\begin{align}
 \int_{0}^{+\infty} \gauss( \mix|u,\sigma^2) d\mix &= \int_{ -u/\sigma }^{+\infty} \gauss( \mix'|0,1) d\mix' \\
 &= 1 - \Phi(-u/\sigma )\\
 &= \Phi(u/\sigma)
\end{align}
\end{comment}


Furthermore, we have
\begin{align*}
  \int_{0}^{+\infty} \mix q(\mix,\vlat|\vmu,\valpha,\vSigma) d\mix 
&=  u_1(\vlat,\vmu,\valpha,\vSigma) \gauss( \vlat| \vmu, \vSigma )  + u_2(\vlat,\vmu,\valpha,\vSigma) q(\vlat|\vmu,\valpha,\vSigma) 
\end{align*} where
$u_1(\vlat,\vmu,\valpha,\vSigma)=\frac{1}{ \valpha^T\vSigma^{-1}\valpha} $ and
$u_2(\vlat,\vmu,\valpha,\vSigma)=\frac{ \left(\vlat-\vmu\right)^T\vSigma^{-1}\valpha -1 }{ \valpha^T\vSigma^{-1}\valpha }$.

\begin{comment}
\begin{align}
  &\int_{0}^{+\infty} \mix q(\mix,\vlat|\vmu,\valpha,\vSigma) d\mix \\
 =&  \int_{0}^{+\infty} \mix \gauss(\vlat|\vmu+\mix\valpha,\vSigma)\expdist(\mix|1) d\mix \\
 =&  \gauss(\vlat|\vmu,\vSigma) \int_{0}^{+\infty}  \mix \exp\crl{  -\half \sqr{  \mix^2 \valpha^T \vSigma^{-1} \valpha - 2\mix \left( \left( \vlat-\vmu \right)^T \vSigma^{-1}\valpha -1 \right) } } d\mix \\
 =&  \gauss(\vlat|\vmu,\vSigma)  \int_{0}^{+\infty} \frac{\sqr{\valpha^T\vSigma^{-1}\valpha  w - \left( \left(\vlat-\vmu\right)^T\vSigma^{-1}\valpha -1 \right) } + \left( \left(\vlat-\vmu\right)^T\vSigma^{-1}\valpha -1\right) }{ \valpha^T\vSigma^{-1}\valpha } \nonumber \\
& \exp\crl{  -\half \sqr{  \mix^2 \valpha^T \vSigma^{-1} \valpha - 2\mix \left( \left( \vlat-\vmu \right)^T \vSigma^{-1}\valpha -1 \right) } } d\mix\\
 =&  \frac{-  \gauss(\vlat|\vmu,\vSigma)}{\valpha^T\vSigma^{-1}\valpha} \exp\crl{  -\half \sqr{  \mix^2 \valpha^T \vSigma^{-1} \valpha - 2\mix \left( \left( \vlat-\vmu \right)^T \vSigma^{-1}\valpha -1 \right) } }  \Big|_{0}^{+\infty}  + \frac{ \left(\vlat-\vmu\right)^T\vSigma^{-1}\valpha -1 }{ \valpha^T\vSigma^{-1}\valpha } \int_{0}^{\infty}  \gauss(\vlat|\vmu+\mix\valpha,\vSigma)\expdist(\mix|1) d\mix \\
 =&  \frac{1}{ \valpha^T\vSigma^{-1}\valpha} \gauss(\vlat|\vmu,\vSigma)  + \frac{ \left(\vlat-\vmu\right)^T\vSigma^{-1}\valpha -1 }{ \valpha^T\vSigma^{-1}\valpha }  q(\vlat|\vmu,\valpha,\vSigma) 
\end{align}
\end{comment}




\end{example}


\begin{theorem}
{\bf Price's Theorem:\\}
Let $h(\vlat):\mathcal{R}^d \mapsto \mathcal{R}$ be a continuously differentiable function that $\nabla h(\vlat)$  has the local ACL property.
Furthermore, $\Unmyexpect{q(\lat)}\sqr{\left| \nabla_{\lat_j} \nabla_{\lat_i} h(\vlat) \right|}<\infty$ for all $i$ and $j$.
Additionally, $\Unmyexpect{q(\mix,\lat)}\sqr{ \left| \nabla_{\lat_j} \crl{ \ve_i^T \vSigma^{-1} \left( \vlat-\vmu-u(\mix)\valpha \right)   h(\vlat)  } \right| } <\infty $ for all $i$ and $j$.
If the regular conditions for Leibniz integral rule are also satisfied, the following gradient identity holds.
\begin{align*}
\nabla_{\Sigma} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) }
= \half \Unmyexpect{q(\lat)}\sqr{  \nabla_{\lat}^2  h(\vlat) }
= \half \Unmyexpect{q(\mix,\lat)}\sqr{  \vSigma^{-1} \left( \vlat-\vmu -u(\mix) \valpha \right)    \nabla_{\lat}^T h(\vlat) } 
%= \half \Unmyexpect{q(\mix,\lat)}\sqr{ \nabla_{\lat} h(\vlat)  \left( \vlat-\vmu -u(\mix)\valpha \right)^T  \vSigma^{-1}  }
\end{align*}
\end{theorem}

\begin{proof}
We can prove that using a similar proof technique used Theorem \ref{claim:price_gauss_lemma}.
\end{proof}


==> content/grad_smg.tex <==
We consider the following  scale mixture of Gaussians.
\begin{align*}
q(\mix,\vlat|\vmu,\vSigma):= &\gauss(\vlat|\vmu , v(\mix)\vSigma) q(\mix) \\
 q(\vlat|\vmu,\vSigma) :=& \int q(\mix,\vlat|\vmu,\vSigma)  d\mix 
\end{align*} where $v(\mix)>0$.


\begin{theorem}
{\bf Bonnet's Theorem:\\}
Let $h(\vlat):\mathcal{R}^d \mapsto \mathcal{R}$ be a continuous function that satisfies the local ACL property.
Furthermore, $\Unmyexpect{q(\lat)}\sqr{\left| \nabla_{\lat_i} h(\vlat) \right|}<\infty$ for all $i$, where  $q(\vlat)$ is a  scale mixture of Gaussians.
If the regular conditions for Leibniz integral rule are also satisfied, the following gradient identity holds.
\begin{align*}
\nabla_{\mu} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) } =&  \Unmyexpect{q(\lat)}\sqr{ \nabla_{\lat} h(\vlat)} 
\end{align*}
\end{theorem}
\begin{proof}
We can prove that using a similar proof technique used Theorem \ref{claim:bonnet_gauss_lemma}.
\end{proof}



\begin{theorem}
{\bf Price's Theorem:\\}
Let $h(\vlat):\mathcal{R}^d \mapsto \mathcal{R}$ be a continuously differentiable function that $\nabla h(\vlat)$  has the local ACL property.
Furthermore, $\Unmyexpect{q(\mix,\lat)}\sqr{\left| v(\mix) \nabla_{\lat_j} \nabla_{\lat_i} h(\vlat) \right|}<\infty$ for all $i$ and $j$.
Additionally, $\Unmyexpect{q(\lat)}\sqr{ \left|  \nabla_{\lat_j} \crl{ \ve_i^T \vSigma^{-1} \left( \vlat-\vmu \right)   h(\vlat)  } \right| } <\infty $ for all $i$ and $j$.
If the regular conditions for Leibniz integral rule are also satisfied, the following gradient identity holds.
\begin{align*}
\nabla_{\Sigma} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) }
= \half \Unmyexpect{q(\mix,\lat)}\sqr{ v(\mix) \nabla_{\lat}^2  h(\vlat) }
= \half \Unmyexpect{q(\lat)}\sqr{  \vSigma^{-1} \left( \vlat-\vmu \right)    \nabla_{\lat}^T h(\vlat) } 
%&= \half \Unmyexpect{q(\lat)}\sqr{  \nabla_{\lat} h(\vlat)  \left( \vlat-\vmu \right)^T  \vSigma^{-1}  }
\end{align*}
\end{theorem}



\begin{proof}

Firstly, note that
\begin{align}
 \Unmyexpect{q(\mix,\lat)}\sqr{ v(\mix) \nabla_{\lat}^2  h(\vlat) }
 &= \Unmyexpect{q(\mix)}\sqr{ v(\mix) \Unmyexpect{q(\lat|\mix)} \sqr{ \nabla_{\lat}^2  h(\vlat) } }\label{eq:smg_eq_1}
\end{align}

Since $\Unmyexpect{q(\mix,\lat)}\sqr{\left| v(\mix) \nabla_{\lat_j} \nabla_{\lat_i} h(\vlat) \right|}<\infty$ and $v(\mix)>0$, we know that
\begin{align*}
\Unmyexpect{q(\mix,\lat)}\sqr{\left| v(\mix) \nabla_{\lat_j} \nabla_{\lat_i} h(\vlat) \right|} 
= \Unmyexpect{q(\mix)}\sqr{ \Unmyexpect{q(\lat|\mix)} \sqr{\left| v(\mix) \nabla_{\lat_j} \nabla_{\lat_i} h(\vlat) \right|} }
= \Unmyexpect{q(\mix)}\sqr{ v(\mix) \Unmyexpect{q(\lat|\mix)} \sqr{\left| \nabla_{\lat_j} \nabla_{\lat_i} h(\vlat) \right|} }
\end{align*} which implies that $\Unmyexpect{q(\lat|\mix)} \sqr{\left| \nabla_{\lat_j} \nabla_{\lat_i} h(\vlat) \right|}<\infty$.

Note that
\begin{align*}
 &\Unmyexpect{q(\lat)}\sqr{ \left|  \nabla_{\lat_j} \crl{ \ve_i^T \vSigma^{-1} \left( \vlat-\vmu \right)   h(\vlat)  } \right| } \\
 =& \Unmyexpect{q(\mix,\lat)}\sqr{ \left|  \nabla_{\lat_j} \crl{ v(\mix) \ve_i^T \left( v(\mix) \vSigma\right)^{-1} \left( \vlat-\vmu \right)   h(\vlat)  } \right| } \\
 =& \Unmyexpect{q(\mix,\lat)}\sqr{ v(\mix) \left|  \nabla_{\lat_j} \crl{  \ve_i^T \left( v(\mix) \vSigma\right)^{-1} \left( \vlat-\vmu \right)   h(\vlat)  } \right| } \\
 =& \Unmyexpect{q(\mix)}\sqr{ v(\mix) \Unmyexpect{q(\lat|\mix)} \sqr{  \left|  \nabla_{\lat_j} \crl{  \ve_i^T \left( v(\mix) \vSigma\right)^{-1} \left( \vlat-\vmu \right)   h(\vlat)  } \right| } }, 
\end{align*} which implies that $\Unmyexpect{q(\lat|\mix)} \sqr{ \left|  \nabla_{\lat_j} \crl{  \ve_i^T \left( v(\mix) \vSigma\right)^{-1} \left( \vlat-\vmu \right)   h(\vlat)  } \right| } <\infty$ since $v(\mix)>0$.


Since $q(\lat|\mix)=\gauss(\vlat|\vmu,v(\mix)\vSigma)$ is a Gaussian, all conditions of Lemma \ref{lemma:stein_gauss_var_price} are satisfied.
By  Lemma \ref{lemma:stein_gauss_var_price}, we have
\begin{align}
  \Unmyexpect{q(\lat|\mix)} \sqr{ \nabla_{\lat}^2  h(\vlat) }
=  \Unmyexpect{q(\lat|\mix)}\sqr{  \left( v(\mix) \vSigma \right)^{-1} \left( \vlat-\vmu \right)    \nabla_{\lat}^T h(\vlat) }  \label{eq:smg_eq_2}
\end{align}

Substituting Eq. \eqref{eq:smg_eq_2} into Eq. \eqref{eq:smg_eq_1},  we have
\begin{align}
& \Unmyexpect{q(\mix,\lat)}\sqr{ v(\mix) \nabla_{\lat}^2  h(\vlat) } \nonumber\\
=& \Unmyexpect{q(\mix)}\sqr{ v(\mix) \Unmyexpect{q(\lat|\mix)}\sqr{  \left( v(\mix) \vSigma \right)^{-1} \left( \vlat-\vmu \right)    \nabla_{\lat}^T h(\vlat) }  } \nonumber\\
=& \Unmyexpect{q(\mix)}\sqr{  \Unmyexpect{q(\lat|\mix)}\sqr{  \vSigma^{-1} \left( \vlat-\vmu \right)    \nabla_{\lat}^T h(\vlat) }  } \nonumber\\
=& \Unmyexpect{q(\lat)}\sqr{   \vSigma^{-1} \left( \vlat-\vmu \right)    \nabla_{\lat}^T h(\vlat) }  \label{eq:smg_eq_3}
\end{align}


Now we can show that $\Unmyexpect{q(\lat)}\sqr{ h(\vlat) }$ exists, due to the following identity.
\begin{align*}
\Unmyexpect{q(\lat)}\sqr{ \ve_i^T\vSigma^{-1} \ve_j  h(\vlat) } = 
  \Unmyexpect{q(\lat)} \sqr{ \ve_i^T \left(  \nabla_{\lat_j} \crl{ \vSigma^{-1} \left( \vlat-\vmu \right)   h(\vlat) } \right)}  -  \Unmyexpect{q(\lat)} \sqr{\ve_i^T \vSigma^{-1} \left( \vlat-\vmu \right)  \nabla_{\lat_j} h(\vlat) } 
\end{align*}  where the first term in the right hand side exists due to $\Unmyexpect{q(\lat)}\sqr{ \left|  \nabla_{\lat_j} \crl{ \ve_i^T \vSigma^{-1} \left( \vlat-\vmu \right)   h(\vlat)  } \right| } <\infty$ and the second term exists due to Eq \eqref{eq:smg_eq_3}.

Since $\Unmyexpect{q(\lat)}\sqr{ h(\vlat) }$ exists, we know that $\Unmyexpect{q(\lat|\mix)}\sqr{ h(\vlat) }$ exists almost everywhere, which is one of the conditions of Lemma
\ref{lemma:stein_gauss_var_reparam}.

Similarly,
since $q(\lat|\mix)=\gauss(\vlat|\vmu,v(\mix)\vSigma)$ is a Gaussian, all conditions of Lemma \ref{lemma:stein_gauss_var_reparam}  are satisfied.
By Lemma \ref{lemma:stein_gauss_var_reparam}, we have
\begin{align*}
 \Unmyexpect{q(\lat|\mix)} \sqr{\left( v(\mix) \vSigma\right)^{-1}  \crl{\left( \vlat-\vmu \right)  \left( \vlat-\vmu \right)^T - v(\mix)\vSigma } \left(v(\mix)\vSigma\right)^{-1}  h(\vlat) } 
=  \Unmyexpect{q(\lat|\mix)}\sqr{ \left(v(\mix) \vSigma\right)^{-1} \left( \vlat-\vmu \right)    \nabla_{\lat}^T h(\vlat) } 
\end{align*}

Therefore, we have
\begin{align}
& \Unmyexpect{q(\lat)}\sqr{   \vSigma^{-1} \left( \vlat-\vmu \right)    \nabla_{\lat}^T h(\vlat) } \nonumber \\
=& \Unmyexpect{q(\mix)}\sqr{  v(\mix) \Unmyexpect{q(\lat|\mix)}\sqr{ \left(v(\mix) \vSigma\right)^{-1} \left( \vlat-\vmu \right)    \nabla_{\lat}^T h(\vlat) } } \nonumber\\
=& \Unmyexpect{q(\mix)}\sqr{  v(\mix) \Unmyexpect{q(\lat|\mix)} \sqr{\left( v(\mix) \vSigma\right)^{-1}  \crl{\left( \vlat-\vmu \right)  \left( \vlat-\vmu \right)^T - v(\mix)\vSigma } \left(v(\mix)\vSigma\right)^{-1}  h(\vlat) } } \nonumber \\
=& \Unmyexpect{q(\mix,\lat)}\sqr{   \vSigma^{-1}  \crl{ u^{-1}(\mix) \left( \vlat-\vmu \right)  \left( \vlat-\vmu \right)^T - \vSigma } \vSigma^{-1}  h(\vlat)  }  \label{eq:smg_eq4}
\end{align}

By the integral rule, we have
\begin{align}
&\nabla_{\Sigma} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) } \nonumber \\
=& \int \nabla_{\Sigma} q(\vlat|\vmu,\vSigma) h(\vlat) d\vlat \\
=& \int \int \sqr{ \nabla_{\Sigma} \gauss(\vlat|\vmu,v(\mix)\vSigma) q(\mix) d\mix } h(\vlat) d\vlat \nonumber\\
=& \half \int \int \sqr{  \vSigma^{-1}  \crl{ u^{-1}(\mix) \left( \vlat-\vmu \right)  \left( \vlat-\vmu \right)^T - \vSigma } \vSigma^{-1}  \gauss(\vlat|\vmu,v(\mix)\vSigma) q(\mix) d\mix } h(\vlat) d\vlat \nonumber \\
=& \half \Unmyexpect{q(\mix,\lat)}\sqr{  \vSigma^{-1}  \crl{ u^{-1}(\mix) \left( \vlat-\vmu \right)  \left( \vlat-\vmu \right)^T - \vSigma } \vSigma^{-1}  h(\vlat)  } \label{eq:smg_eq5} 
\end{align}

Finally, by Eq. \eqref{eq:smg_eq_3} , \eqref{eq:smg_eq4}, and \eqref{eq:smg_eq5}, we have
\begin{align*}
\nabla_{\Sigma} \Unmyexpect{q(\lat)} \sqr{ h(\vlat) }  
= \half \Unmyexpect{q(\lat)}\sqr{   \vSigma^{-1} \left( \vlat-\vmu \right)    \nabla_{\lat}^T h(\vlat) }
= \half \Unmyexpect{q(\mix,\lat)}\sqr{ v(\mix) \nabla_{\lat}^2  h(\vlat) } 
\end{align*}


\end{proof}


\begin{corollary}
If $v(\mix)$ has the following property, 
\begin{align*}
\int v(\mix) q(\mix,\vlat|\vmu,\valpha,\vSigma) d\mix  = \sum_j^k v_j(\vlat,\vmu,\vSigma) \hat{q_j}(\vlat),
\end{align*}  where $\hat{q}_i(\vlat)$ is a (normalized) distribution and $k$ is finite,
the following identity also holds.
\begin{align*}
 \nabla_{\Sigma} \Unmyexpect{q(\lat)} \sqr{  h(\vlat) }  
=  \half \Unmyexpect{q(\mix,\lat)}\sqr{ v(\mix) \nabla_{\lat}^2  h(\vlat) }
= \half \sum_{j}^k  \Unmyexpect{\hat{q_j}(\lat)}\sqr{ v_j(\vlat,\vmu,\vSigma) \nabla_{\lat}^2 h(\vlat)}  
\end{align*}
\end{corollary}



\begin{example}
 

A concrete example is the multivariate Student's t-distribution with fixed degree of freedom $2\alpha$.
We consider a case when $\alpha>1$, since the variance exists in this case.
\begin{align*}
q(\mix,\vlat|\vmu,\vSigma):= & \gauss(\vlat|\vmu ,\mix \vSigma) \IG(\mix|\alpha,\alpha)  \\
 q(\vlat|\vmu,\vSigma) := &  \int q(\mix,\vlat|\vmu,\vSigma)  d\mix \\
=&  \mathrm{det}\left(\pi \vSigma \right)^{-1/2}  \frac{   \Gamma(a+d/2)  \left(   2a + \left(\vlat-\vmu\right)^T \vSigma^{-1}  \left(\vlat-\vmu\right)    \right)^{-a-d/2} }{   \Gamma(a)     \left( 2a\right)^{-a} } .
\end{align*} where $v(\mix)=\mix>0$ since $\mix$ is generate from inverse Gamma distribution $\IG(\mix|\alpha,\alpha)$.

When $\alpha>1$,  we have
\begin{align*}
  \int \mix q(\mix,\vlat|\vmu,\valpha,\vSigma) d\mix 
&=  v_1(\vlat,\vmu,\vSigma) q(\vlat|\vmu,\vSigma) 
\end{align*} where
$v_1(\vlat,\vmu,\vSigma):=\frac{a}{(a+d/2-1)} \left(1 + (2a)^{-1} \left( \vlat-\vmu \right)^T \vSigma^{-1} \left( \vlat-\vmu \right) \right)$.


\end{example}

